WikiRank: Improving Keyphrase Extraction Based on Background Knowledge

Keyphrase is an efficient representation of the main idea of documents. While background knowledge can provide valuable information about documents, they are rarely incorporated in keyphrase extraction methods. In this paper, we propose WikiRank, an unsupervised method for keyphrase extraction based on the background knowledge from Wikipedia. Firstly, we construct a semantic graph for the document. Then we transform the keyphrase extraction problem into an optimization problem on the graph. Finally, we get the optimal keyphrase set to be the output. Our method obtains improvements over other state-of-art models by more than 2% in F1-score.

==> ConceptTableTotal.tex <==
\begin{table}[!ht]
\begin{center}
\begin{tabularx}{\columnwidth}{|l|l|X|}
    \hline
    No.&Concept&Frequency\\\hline
    1&Cattle & 6\\\hline
    2&Disease & 6\\\hline
    3&Great Britain & 4\\\hline
    4&Bovine spongiform encephalopathy & 4\\\hline
    5&Risk & 3\\\hline
    6&United States Department & 3\\
    &of Agriculture &\\\hline
    7&John Lowry Gourlay & 2\\\hline
    8&Sheep milk & 2 \\\hline
    9&Last year & 2 \\\hline
    10&Export & 2\\\hline
    11&Market price & 2 \\\hline
    12&Encephalopathy & 2 \\ \hline
    13&Human &2 \\ \hline 
    14&Committee &2 \\ \hline
    15&Percentage  & 2 \\\hline
    16&Health & 2 \\ \hline 
    17&Brain  & 1 \\\hline
    18&Doughnut & 1\\\hline
    19&Spinal cord & 1\\\hline
    20&British Empire & 1\\\hline 
    21&Educational assessment & 1\\\hline
    22&Mutation & 1\\\hline
    23&Food chain & 1\\\hline
    24&Minister of Agriculture (Canada) & 1\\\hline
    25&Infection & 1\\\hline
    26&Israel & 1\\\hline
    27&Margaret, Maid of Norway & 1\\\hline
    28&Suspicion & 1\\\hline
    29&London, Ontario & 1\\\hline
    30&University of Oxford & 1\\\hline
    31&European Union & 1\\\hline
    32&Bacteria & 1\\\hline
    33&Frozen bovine semen & 1\\\hline
    34&Nick Southwood & 1\\\hline
    35&Plant pathology & 1\\\hline
    36&Science & 1\\\hline
    37&Case study & 1\\\hline
    38&Agriculture & 1\\\hline
    39&Public&1\\\hline
\end{tabularx}
\caption{Concepts Extracted from the Sameple Document }
 \end{center}
\end{table}
